Salem/Pisot Numbers in the Weyl Spectrum

n this article, we define orbit data for birational maps of $\mathbf{P}^2(\mathbb{C})$ and show that this data uniquely determines the dynamical degree by providing minimal polynomials for dynamical degrees in terms of orbit data. Leveraging this relationship, we recursively identify all Salem and Pisot numbers that appear in the Weyl spectrum of the union of the Coxeter groups $W_n$ associated with $E_n$ and the set of all dynamical degrees of birational maps of $\mathbf{P}^2(\mathbb{C})$. Furthermore, we demonstrate that all accumulation points of Pisot numbers less than or equal to 2 are present in the Weyl spectrum.

==> intro.tex <==
A Pisot number $\tau$ is an algebraic integer greater than $1$ whose Galois conjugates all have modulus $\lneq1$. A Salem number $\lambda$, defined by Salem \cite{Salem:1945}, is an algebraic integer whose minimal polynomial is of degree at least $4$, and all of whose Galois conjugates, except $\lambda$ and $\lambda^{-1}$, have modulus $1$. Salem and Pisot numbers are closely related in the sense that every Pisot number is a limit of a sequence of Salem numbers. However, it is not known that every limit of a sequence of distinct Salem numbers is a Pisot number. Salem and Pisot numbers have appeared in many different areas of Mathematics. (See \cite{Erdos:1939, Boyd:1977, Sury:1992, HironakaE:2001, Tanigawa:2004}.) For a detailed history, we refer to a comprehensive survey by Smyth \cite{Smyth:2015}.


Salem and Pisot numbers appear in Dynamical Systems. Diller and Favre \cite{Diller-Favre:2001} and Blanc and Cantat \cite{blancdynamical} showed that the exponential growth rate of the algebraic degree of a birational map on $\mathbf{P}^2(\mathbb{C})$ under iteration is given by either a Salem or Pisot number. This exponential growth rate of the degree is called \textit{the dynamical degree}. However, not every Salem/Pisot number can be realized. Blanc and Cantat \cite{blancdynamical} show that infinitely many Pisot numbers greater than the golden ratio cannot be realized as the dynamical degree of a birational map on $\mathbf{P}^2(\mathbb{C})$. 

According to Diller and Favre \cite{Diller-Favre:2001}, McMullen \cite{McMullen:2007}, Uehara \cite{Uehara:2010}, Kim \cite{Kim:2023}, and Blanc and Cantat \cite{blancdynamical}, we know that the set of all dynamical degrees of birational maps on $\mathbf{P}^2(\mathbb{C})$ is identical to the Weyl spectrum, the closure of the set of spectral radii of elements in Coxeter group associated with $E_n, n\ge 10$. The main goal of this article is to determine Salem and Pisot numbers in the Weyl spectrum and study their properties as dynamical degrees of birational maps on $\mathbf{P}^2(\mathbb{C})$.

\vspace{1ex}
 
 The Coxeter group $W_n, n\ge 4$, associated with $E_n$ diagram in Figure \ref{fig:coxetergraph} is the group with generators $s_i$'s and relations \[ (s_i s_j)^{m_{i,j}} = 1 \qquad \text{where}\ \ m_{i,j} \ =\   \left\{ \ \begin{aligned} & 1 \ \ \text{ if } i=j,\\ &  2 \ \ \text{ if there is no edge joining } s_i \text{ and } s_j, \\ & 3 \ \ \text{ if there is an edge joining } s_i \text{ and } s_j. \\ \end{aligned} \right. \]


 \begin{figure}[h]
\centering
\includegraphics{Figure1.pdf}
\caption{Coxeter Graph $E_n$ \label{fig:coxetergraph} }
\end{figure}
For $\omega \in W_n$, we say $\omega$ is \textit{essential} if, for all $\rho \in W_n$, the conjugate $\rho \omega \rho^{-1}$ is not an element of a proper subgroup generated by $s_i$, where $ i \in I \subsetneq \{0, 1, \dots, n-1\}$. The Coxeter group $W_n$ has a faithful reflection representation on a vector space $V_n$ with the inner product $B_n(\alpha_i,\alpha_j) = -2 \cos (\pi/m_{ij})$ on the basis $\{\alpha_i\}$ dual to $\{s_i\}$. Let $\lambda(\omega)$ denote the leading eigenvalue of $\omega|_{V_n}$. McMullen \cite{McMullen:2002} showed that if $\omega \in W_n, n\ge 10$ is essential, then the spectral radius $\lambda(\omega)$ is always greater than or equal to $\lambda_{10}$. The Salem number $\lambda_{10} \approx 1.176$, known as Lehmer's number, has the minimal polynomial:   \[ L(t) = t^{10} +t^9-t^7-t^6-t^5-t^4-t^3+t+1. \]

Let us define $\Lambda_{S,W}$ as the set of all spectral radii of essential elements in $W_n, n\ge 10$: \[ \Lambda_{S,W} := \{ \lambda(\omega): \omega \text{ is an essential element in } W_n, n\ge 10 \}. \]  Since every element in $W_n, n\le 9$ has spectral radius equal to $1$, we have \[  \{ \lambda(\omega): \omega\in W_n, n\ge 4 \} = \{1\} \cup \Lambda_{S,W}.\]
We denote the closure of all spectral radii of $W_n, n\ge 4$ as the Weyl spectrum, $ \Lambda_W$: \[ \Lambda_W \ =\  \{1\} \cup \overline{\Lambda_{S,W}}.\]

 It is known \cite{Lakatos:2001, Lakatos:2010} that the spectral radius of $\omega \in W_n$ is either $1$, a reciprocal quadratic integer, or a Salem number. A reciprocal quadratic integer $q_n$ is an algebraic integer whose minimal polynomial is $1- n t + t^2$ for some integer $n$. By Blanc and Cantat \cite{blancdynamical}, every positive reciprocal quadratic integer is realized as a spectral radius of an element of $W_n$. The smallest positive reciprocal quadratic integer greater than $1$ is $q_3 \approx 2.618$. This quadratic integer, $q_3$, is realized as a spectral radius of an element $\omega_q\in W_{10}$ where 
\[  \omega_q =s_1   s_7   s_9   \kappa_{2,3,4}   \kappa_{2,5,6}   \kappa_{2,8,10}   \kappa_{3,4,5}   \kappa_{6,8,10}, \]
\[
  \kappa_{i,j,k} = \rho_{1,i}   \rho_{2,j}  \rho_{3,k}   s_0    \rho_{1,i}   \rho_{2,j}  \rho_{3,k}, \qquad\text{and} \qquad \rho_{i,j} = s_i s_{i+1} \cdots s_{j-1}. \]
On the other hand, not every Salem number is realized as a spectral radius of an element of $W_n$. However, McMullen \cite{McMullen:2002} showed that the smallest known Salem number, $\lambda_{10}$, is indeed realized as a spectral radius of the Coxeter element in $W_{10}$. 
Thus, $\lambda_{10}$ is the smallest number greater than $1$ in $\Lambda_W$.
 
 \vspace{1ex}
 As noted above, any limit of Salem numbers is either a Salem or Pisot number. Consequently, the Weyl spectrum consists of $1$, Salem numbers, and Pisot numbers. Let us denote by $\Lambda_{P,W}$ the set of limit points of $\Lambda_{S,W}$:
 \[ \Lambda_W = \{1\} \cup \Lambda_{S,W} \cup \Lambda_{P,W}. \]
 
 \vspace{1ex}
 On the other hand, the Weyl spectrum $\Lambda_W$ is realized as the set of dynamical degrees of birational maps on $\mathbf{P}^2(\mathbb{C})$. Consider a birational transformation $f=[f_1:f_2:f_3]$ on $\mathbf{P}^2(\mathbb{C})$, where $f_1, f_2$ and $f_3$ are polynomials of degree $d$ without a non-constant common factor. The degree of $f$ is given by the common degree $d$ of the coordinate polynomials, and the dynamical degree $\lambda(f)$ is defined by \[ \lambda(f) \ =\ \lim_{n \to \infty} (\deg f^n)^{1/n}. \]
 Because of possible common factors in the $n$-fold composition of $f$, we have $\deg (f^n) \le (\deg f)^n$, and thus, computing the dynamical degree of a given birational map is a challenging task. For a given birational map $f \in \bptwo$, Diller and Favre \cite{Diller-Favre:2001} showed that there is always a rational surface $X$, obtained by blowing up $\mathbf{P}^2(\mathbb{C})$ along a finite set of points, such that the induced map $F:X \to X$ satisfies \[ \lambda(F) = \lambda(f) = \rho(F_*) \] where $\rho$ denotes the spectral radius and $F_*$ is the induced linear map on $\pic(X)$. Also, by Diller and Favre \cite{Diller-Favre:2001} and Blanc and Cantat \cite{blancdynamical}, we have:
 \begin{thm}\cite{Diller-Favre:2001, blancdynamical}\label{inT:ddeg} Suppose $f \in \bptwo$ is a birational transformation with a dynamical degree $\lambda(f) >1$. Then we have one of the following:
 \begin{itemize}
 \item $f$ is birationally equivalent to an automorphism, and the dynamical degree $\lambda(f)$ is either a Salem number or a reciprocal quadratic integer.
 \item $f$ is not birationally equivalent to an automorphism, and the dynamical degree $\lambda(f)$ is a Pisot number.   
 \end{itemize}
 \end{thm}
 
Let us denote by $\Lambda_\mathbb{C}$ the set of all dynamical degrees of birational maps on $\mathbf{P}^2(\mathbb{C})$. 
Let us also denote by $\Lambda_{S, \mathbb{C}} \subset \Lambda_\mathbb{C}$ the set of all dynamical degrees of birational maps equivalent to an automorphism, and by $\Lambda_{P, \mathbb{C}} \subset \Lambda_\mathbb{C}$ the set of all dynamical degrees of birational maps that are not equivalent to an automorphism. Then, by Theorem \ref{inT:ddeg}, the set $\Lambda_{S, \mathbb{C}}$ consists of $1$, reciprocal quadratic integers, and Salem numbers, and the set $\Lambda_{P, \mathbb{C}}$ consists of Pisot numbers. 
By Nagata \cite{Nagata, Nagata2}, if $F$ is an automorphism on a rational surface $X$ over $\mathbb{C}$ with infinite order, then the induced action $F_*$ on $\text{Pic}(X)$ is an element of $W_n$, where $n+1$ is the Picard rank of $X$. Thus we have $\Lambda_{S, \mathbb{C}} \subset \Lambda_{S, W}$. McMullen \cite{McMullen:2007}, Uehara \cite{Uehara:2010}, and Kim \cite{Kim:2023} show that, in fact,
\[ \Lambda_{S, \mathbb{C}} = \Lambda_{S, W}. \] 
Also, Blanc and Cantat \cite{blancdynamical} show that the dynamical spectrum $\Lambda_\mathbb{C}$ is well-ordered and closed. It follows that \[  \Lambda_W = \Lambda_\mathbb{C}.\] To simplify our notations, let us use $\Lambda_{S}$ for both $\Lambda_{S, W}$ and $\Lambda_{S, \mathbb{C}}$. 

\begin{rem}
Since $\Lambda_W = \Lambda_\mathbb{C}$, the closure of Salem numbers in the Weyl spectrum consists of both Pisot and Salem numbers. Thus, in principle, there could be a Salem number in $\Lambda_{P,W} \setminus \Lambda_{S,W}$. However, by combining the identities $\Lambda_{S, \mathbb{C}} = \Lambda_{S, W}$ and $\Lambda_W = \Lambda_\mathbb{C}$ with the result of Blanc and Cantat \cite{blancdynamical}, we conclude that if a Salem number $\lambda$ is in $\Lambda_{P,W}$, then $\lambda$ must also lie in $\Lambda_S$. Consequently, there is no Salem number in $\Lambda_{P,W} \setminus \Lambda_{S,W}$.
%(See Proposition \ref{P:n1}.)
\end{rem}


\vspace{1ex}
In this article, using theories from the Coxeter group and birational maps on $\mathbf{P}^2(\mathbb{C})$, we show the following:


\begin{thma}
The Weyl spectrum $\Lambda_W$ is given by 
\[ \Lambda_W =\{ \rho(\chi_{M, \bar n}): M \in \bigcup_d (\mathcal{M}_d \cup  \mathcal{M}'_d), \bar n \in \mathbb{N}^k, k = |M|-1, d\ge 2 \} \]
where $\rho$ denotes the largest real root, $|M|$ denotes the size of $M$,  $\chi$ is defined in (\ref{E:charpoly}), $\mathcal{M}_d, d\ge 2 $ is given recursively by the Theorem \ref{T:allbase}, and $  \mathcal{M}'_d, d\ge 2$ is defined in (\ref{E:setM}).
\end{thma}

For a birational map $f \in \bptwo$, there is the set $\mathcal{E}(f)$ of exceptional curves mapped to a point and the set $\mathcal{I}(f)$ of points of indeterminacy. Any irreducible curve in $\mathcal{E}(f)$ maps to a point under $f$.  Let us define $\mathcal{E}^*(f)$ as the set of exceptional curves mapped back to a curve:
\[ \mathcal{E}^*(f) = \{ C \in \mathcal{E}(f) : f^{n} (C) \in \mathcal{I}(f), \ \ \dim f^{n+1}(C) =1, n\ge 1 \} \]
For each $C_i \in \mathcal{E}^*(f)$, let $n_i$ be the smallest number of iterations $n$ such that $\dim f^{n+1}(C_i) =1$. We call the ordered tuple $(n_1, \dots, n_k)$, where $k=|\mathcal{E}^*(f)|$, the orbit lengths of $f$. 
In Section \ref{S:birational}, we define \textit{the orbit data} of $f$ as the numerical data obtained by orbits of curves in $\mathcal{E}^*(f)$. We show that the dynamical degree increases with respect to the orbit lengths. 
\begin{thmb}
Let $f$ and $g$ are birational maps on $\mathbf{P}^2(\mathbb{C})$. Suppose the orbit data of $f$ and $g$ are distinct, given by $\mathcal{O}(f)=(M, (n_1, \dots, n_k))$ and $\mathcal{O}(g)=(M, (n'_1, \dots, n'_k))$ respectively. Assume the following conditions hold:
\begin{enumerate}
\item  $n_i \le n'_i$ for all $i=1, \dots, k$,
\item $n_i \ne n'_i$ for some $i$, 
\item $\lambda(f)>1$.
\end{enumerate}
Then $\lambda(g) \gneq \lambda(f)$. 
\end{thmb}

The smallest accumulation point of Pisot numbers is the golden ratio. With the construction provided by Diller \cite{Diller:2011}, we show: 
\begin{thmc}
All Pisot numbers smaller than or equal to the golden ratio are realized as dynamical degrees of birational maps on $\mathbf{P}^2(\mathbb{C})$. 
\end{thmc}

This article is organized as follows: In Section \ref{S:birational}, we discuss basic facts about birational maps on $\mathbf{P}^2(\mathbb{C})$ and define orbit data for these maps. In Section \ref{S:coxeter}, we explore the properties of the Coxeter group and give a formula for the characteristic polynomial of any element within the group. The proof of Theorem A is in Section \ref{S:sp}, and the proof of Theorem B is in Section \ref{S:spec}, and Section \ref{S:pisot} lists orbit data corresponding to Pisot numbers smaller than or equal to the golden ratio, including the proof of Theorem C. 



==> salem.tex <==
\subsection{Properties of Spectral radii}\label{SS:pspec}

\begin{prop}\label{P:pisot}
Suppose $\chi(t)$ is the characteristic polynomial (up to a product of cyclotomic polynomials) of an element with orbit data $(M, (n_1,n_2, \dots, n_k))$ defined in (\ref{E:charpoly}). For any non-empty subset $I \in \{1, \dots, k\}$, we have \[ \chi(t) = t^{\sum_{i \in I} n_i} \psi(t) + \phi(t), \qquad \text{where} \]


the coefficient of $t^{n_I} = t^{\sum_{i\in I} n_i} $ in $\chi(t)$ is a Pisot polynomial. 
\end{prop}

\begin{proof}
\end{proof}

%The Pisot polynomial of the above proposition only depends on $n_i, i \not\in I$, 
%
%\begin{lem}\label{L:largepisot}
%For given positive integers $n_{2}, \dots n_{k}$, let $\lambda_p$ be the largest real root of the coefficient 
%\end{lem}



\begin{prop}\label{P:mono}
Suppose $\omega$ and $\omega'$ have distinct orbit data $(M, (n_1, \dots, n_k))$ and $(M, (n'_1, \dots, n'_k))$ respectively. If $n_i \le n'_i$ for all $i=1, \dots, k$, and $\lambda(\omega)>1$ then $\lambda(\omega) \lneq \lambda(\omega')$. 
\end{prop}

\begin{proof}
It is enough to show that case $n'_1 = n_1+1$ and $n'_i = n_i$ for $i\ge 2$. Let $t_\star>1$ be the spectral radius of $\omega$. With (\ref{E:charpoly}), we see that $t_\star$ is the unique real root $>1$ of \[ \sum_I t^{N-n_I} \det M_I = t^{n_1} \psi(t) + \phi(t),   \]
where $\psi(t)$ and $\phi(t)$ are polynomials independent to $n_1$ given by 
\[ \psi(t) \ =\  \sum_{ 1 \in I} t^{(N-n_1)-n_I} \det M_I , \quad \phi(t) \ =\  \sum_{ 1 \not \in I} t^{N-n_I} \det M_I.\]
Thus we have \[ t_\star^{n_1} \psi(t_\star) = - \phi(t_{\star}), \]
\[t^{n_1} \psi(t) + \phi(t) < 0 \ \ \text{for}\ \ t>t_\star, \qquad \text{and} \qquad t^{n_1} \psi(t) + \phi(t) > 0 \ \ \text{for}\ \ 1< t < t_\star. \]
\end{proof}

\begin{lem}\label{L:d3}
At least three $d_i$'s are bigger than $d/3$.
\end{lem}

\begin{prop}\label{P:everything}
\end{prop}


